Vehicle Teleoperation: Performance Assessment of SRPT Approach Under State Estimation Errors

Vehicle teleoperation has numerous potential applications, including serving as a backup solution for autonomous vehicles, facilitating remote delivery services, and enabling hazardous remote operations. However, complex urban scenarios, limited situational awareness, and network delay increase the cognitive workload of human operators and degrade teleoperation performance. To address this, the successive reference pose tracking (SRPT) approach was introduced in earlier work, which transmits successive reference poses to the remote vehicle instead of steering commands. The operator generates reference poses online with the help of a joystick steering and an augmented display, potentially mitigating the detrimental effects of delays. However, it is not clear which minimal set of sensors is essential for the SRPT vehicle teleoperation control loop. This paper tests the robustness of the SRPT approach in the presence of state estimation inaccuracies, environmental disturbances, and measurement noises. The simulation environment, implemented in Simulink, features a 14-dof vehicle model and incorporates difficult maneuvers such as tight corners, double-lane changes, and slalom. Environmental disturbances include low adhesion track regions and strong cross-wind gusts. The results demonstrate that the SRPT approach, using either estimated or actual states, performs similarly under various worst-case scenarios, even without a position sensor requirement. Additionally, the designed state estimator ensures sufficient performance with just an inertial measurement unit, wheel speed encoder, and steer encoder, constituting a minimal set of essential sensors for the SRPT vehicle teleoperation control loop.

==> sections/06_metadata.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% optional
%\supplementary{The following supporting information can be downloaded at:  \linksupplementary{s1}, Figure S1: title; Table S1: title; Video S1: title.}

% Only for the journal Methods and Protocols:
% If you wish to submit a video article, please do so with any other supplementary material.
% \supplementary{The following supporting information can be downloaded at: \linksupplementary{s1}, Figure S1: title; Table S1: title; Video S1: title. A supporting video article is available at doi: link.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\authorcontributions{For research articles with several authors, a short paragraph specifying their individual contributions must be provided. The following statements should be used ``Conceptualization, X.X. and Y.Y.; methodology, X.X.; software, X.X.; validation, X.X., Y.Y. and Z.Z.; formal analysis, X.X.; investigation, X.X.; resources, X.X.; data curation, X.X.; writing---original draft preparation, X.X.; writing---review and editing, X.X.; visualization, X.X.; supervision, X.X.; project administration, X.X.; funding acquisition, Y.Y. All authors have read and agreed to the published version of the manuscript.'', please turn to the  \href{http://img.mdpi.org/data/contributor-role-instruction.pdf}{CRediT taxonomy} for the term explanation. Authorship must be limited to those who have contributed substantially to the work~reported.}
\authorcontributions{Conceptualization, methodology, software, validation, data curation, formal analysis, investigation, visualization, writing---original draft preparation, writing---review and editing, J.P.;
Supervision, methodology, formal analysis, validation, project administration, writing---review and editing, M.V.;
Supervision, project administration, writing---review and editing, E.S.;
Resources, funding acquisition, F.C. All authors have read and agreed to the published version of the manuscript.
}

\funding{\hl{This research} received no external funding.} 
 %MDPI: Please check the accuracy of funding data and any other information carefully.
 %Author: I confirm, no funding information needs to be added for this work.

%\institutionalreview{In this section, you should add the Institutional Review Board Statement and approval number, if relevant to your study. You might choose to exclude this statement if the study did not require ethical approval. Please note that the Editorial Office might ask you for further information. Please add “The study was conducted in accordance with the Declaration of Helsinki, and approved by the Institutional Review Board (or Ethics Committee) of NAME OF INSTITUTE (protocol code XXX and date of approval).” for studies involving humans. OR “The animal study protocol was approved by the Institutional Review Board (or Ethics Committee) of NAME OF INSTITUTE (protocol code XXX and date of approval).” for studies involving animals. OR “Ethical review and approval were waived for this study due to usage of a simulated driving environment and not a real vehicle, which ensures no-risk to the volunteers.” OR “Not applicable” for studies not involving humans or animals.}

\institutionalreview{Not applicable.}

\informedconsent{Informed consent was obtained from all subjects involved in the study.

%Written informed consent for publication must be obtained from participating patients who can be identified (including by the patients themselves). Please state ``Written informed consent has been obtained from the patient(s) to publish this paper'' if applicable.
}

\dataavailability{Not applicable.} 

\acknowledgments{The authors are grateful to all the 18 volunteer drivers for their participation in the experimental campaign. Their identities are anonymized.
}

\conflictsofinterest{The authors declare no conflict of \hl{interest}.}   %MDPI: please check if the manuscript has Appendix, has Appendix tex in the zip. %Author: No appendix is required, file has been removed now. Thank you for your observation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Optional
%\sampleavailability{Samples of the compounds ... are available from the authors.}

%% Only for journal Encyclopedia
%\entrylink{The Link to this entry published on the encyclopedia platform.}

\abbreviations{Abbreviations}{
The following abbreviations are used in this manuscript:\\

\noindent 
\begin{tabular}{@{}ll}
SRPT & Successive Reference-Pose Tracking\\
NMPC & Non-linear Model-Predictive Control\\
FOV & Field Of View\\
ODE & Ordinary Differential Equation\\
DOF & Degree of Freedom\\
IMU & Inertial Measurement Unit
\end{tabular}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
%% Optional
\appendixtitles{no} % Leave argument "no" if all appendix headings stay EMPTY (then no dot is printed after "Appendix A"). If the appendix sections contain a heading then change the argument to "yes".
\appendixstart
\appendix
\section[\appendixname~\thesection]{}
\subsection[\appendixname~\thesubsection]{}
The appendix is an optional section that can contain details and data supplemental to the main text---for example, explanations of experimental details that would disrupt the flow of the main text but nonetheless remain crucial to understanding and reproducing the research shown; figures of replicates for experiments of which representative data are shown in the main text can be added here if brief, or as Supplementary Data. Mathematical proofs of results not central to the paper can be added as an appendix.

\begin{table}[H] 
\caption{This is a table caption.\label{tab5}}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{tabularx}{\textwidth}{CCC}
\toprule
\textbf{Title 1}	& \textbf{Title 2}	& \textbf{Title 3}\\
\midrule
Entry 1		& Data			& Data\\
Entry 2		& Data			& Data\\
\bottomrule
\end{tabularx}
\end{table}

\section[\appendixname~\thesection]{}
All appendix sections must be cited in the main text. In the appendices, Figures, Tables, etc. should be labeled, starting with ``A''---e.g., Figure A1, Figure A2, etc.
\fi

==> sections/09-bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/JaiPrakash.png}}]%
{Jai Prakash}
received the M.S. degree in Mechanical Engineering from the Politecnico di Milano, Italy in 2018. He is currently a PhD candidate in the Mechanical Engineering Department of Politecnico di Milano. His research interests include computer-vision, robotics, vehicle dynamics and vehicle teleoperation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/mic.jpg}}]%
{Michele Vignati} (member IEEE) received his master degree (2013) and PhD (2017) in mechanical engineering in Mechanical Department of Politecnico di Milano with thesis on control strategies for distributed powertrain of hybrid and electric vehicles. From 2019 he is Senior Assistant Professor (RTDB) in the research field of applied mechanics. In particular, he focuses on mechanical systems dynamics and control applied in the automotive field of which he has more than 40 publications in international journals and conferences. In 2018 he won the best paper award for a paper presented at the AVEC18 international conference. He worked on tire dynamics and modelling in cooperation with Pirelli while in the last years he is working in autonomous driving field. His expertise goes from vehicle and tire dynamics to vehicle control systems and energy management.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/edo.png}}]%
{Edoardo Sabbioni}
received his PhD in Mechanical Systems Engineering in 2007 and currently works as Associate Professor at the Department of Mechanical Engineering of Politecnico di Milano. His main research activities are in the field of stability, dynamics and control of mechanical systems, with applications to road and rail vehicles. He is also involved in research activities within the fields of aerodynamics and mechatronics. More in particular, he carried out numerical-experimental researches concerned with active safety of vehicles, design of control systems to improve vehicle handling and ride comfort, design of HiL (Hardware-in-the-Loop) test benches, electric and hybrid electric vehicles, autonomous and connected vehicle, “smart” tires technology, cross wind on road/rail vehicles. He is an author of more than 140 scientific publications, most of which published on peer-reviewed journals or presented at international conferences and he is a member of the Editorial Board of Shock and Vibration.

During his research activity, he cooperated and still cooperates with the main Italian automotive/railway industries and he was involved in several Italian and EC funded projects.
\end{IEEEbiography}

%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]%{Figures/cheli.jpg}}]%
%{Federico Cheli}
%received the M.S. degree in mechanical engineering from the Politecnico di Milano, Milano, Italy, in 1981. He is currently a Full Professor at the Department of Mechanical Engineering, Politecnico di Milano and author of more than 380 publications on international journals and conferences. His scientific activity concerns research on vehicle performance, handling and comfort problems, active control, ADAS, and electric and autonomous vehicles. He is a member of the editorial board of the International Journal of Vehicle Performance and International Journal of Vehicle Systems Modeling and Testing.
%\end{IEEEbiography}

==> sections/100_bibiliography.tex <==

\begin{thebibliography}{1}

\bibitem{ams}
{\it{Mathematics into Type}}, American Mathematical Society. Online available: 

\bibitem{oxford}
T.W. Chaundy, P.R. Barrett and C. Batey, {\it{The Printing of Mathematics}}, Oxford University Press. London, 1954.

\bibitem{lacomp}{\it{The \LaTeX Companion}}, by F. Mittelbach and M. Goossens

\bibitem{mmt}{\it{More Math into LaTeX}}, by G. Gr\"atzer

\bibitem{amstyle}{\it{AMS-StyleGuide-online.pdf,}} published by the American Mathematical Society

\bibitem{Sira3}
H. Sira-Ramirez. ``On the sliding mode control of nonlinear systems,'' \textit{Systems \& Control Letters}, vol. 19, pp. 303--312, 1992.

\bibitem{Levant}
A. Levant. ``Exact differentiation of signals with unbounded higher derivatives,''  in \textit{Proceedings of the 45th IEEE Conference on Decision and Control}, San Diego, California, USA, pp. 5585--5590, 2006.

\bibitem{Cedric}
M. Fliess, C. Join, and H. Sira-Ramirez. ``Non-linear estimation is easy,'' \textit{International Journal of Modelling, Identification and Control}, vol. 4, no. 1, pp. 12--27, 2008.

\bibitem{Ortega}
R. Ortega, A. Astolfi, G. Bastin, and H. Rodriguez. ``Stabilization of food-chain systems using a port-controlled Hamiltonian description,'' in \textit{Proceedings of the American Control Conference}, Chicago, Illinois, USA, pp. 2245--2249, 2000.

\end{thebibliography}
